Byzantine Resilient Distributed Multi-Task Learning

Distributed multi-task learning provides significant advantages in multi-agent networks with heterogeneous data sources where agents aim to learn distinct but correlated models simultaneously.However, distributed algorithms for learning relatedness among tasks are not resilient in the presence of Byzantine agents. In this paper, we present an approach for Byzantine resilient distributed multi-task learning. We propose an efficient online weight assignment rule by measuring the accumulated loss using an agent's data and its neighbors' models. A small accumulated loss indicates a large similarity between the two tasks. In order to ensure the Byzantine resilience of the aggregation at a normal agent, we introduce a step for filtering out larger losses. We analyze the approach for convex models and show that normal agents converge resiliently towards the global minimum.Further, aggregation with the proposed weight assignment rule always results in an improved expected regret than the non-cooperative case. Finally, we demonstrate the approach using three case studies, including regression and classification problems, and show that our method exhibits good empirical performance for non-convex models, such as convolutional neural networks.

==> convergence.tex <==
\section{Convergence Analysis}
Suppose the loss function $\ell_k$ is a $m$-strongly convex function and has $L$-Lipschitz continuous gradient for every $k$. As a result, the same condition holds for $r_k$.
Hence, $r_k$ has a unique minimizer $\theta^*$ with $r_k^* = r_k(\theta^*)$. In the following, we prove the convergence of the proposed update rule and weight assignment rules, using fixed stepsizes $\mu_k = \mu_l = \mu$.
% Given the update rule, we have
% \begin{equation*}
% \begin{aligned}
%   &  \|\theta_{k,i+1} - \theta_k^*\|_2^2 = \|\sum_{l \in \mathcal{N}_k} a_{lk}(i) (\theta_{l,i} - \mu \nabla_{\theta_l} \ell_l^i(\theta_{l,i})) - \theta_k^*\|_2^2 \\
%     &= \|\sum_{l \in \mathcal{N}_k} a_{lk}(i) (\theta_{l,i} - \theta_k^*)\|_2^2 + \mu^2 \|\sum_{l \in \mathcal{N}_k} a_{lk}(i)  \nabla_{\theta_l} \ell_l^i(\theta_{l,i})) \|_2^2 - 2 \mu \left(\sum_{l \in \mathcal{N}_k} a_{lk}(i)  \nabla_{\theta_l} \ell_l^i(\theta_{l,i}) \right)^\top \left(\sum_{l \in \mathcal{N}_k} a_{lk}(i) (\theta_{l,i} - \theta_k^*) \right)\\
% \end{aligned}
% \end{equation*}
% Given Jensen's inequality and taking expectations of  the inequality, we have 
% $$\mathbb{E} [\| \sum_{l \in \mathcal{N}_k} a_{lk}(i) (\theta_{l,i} - \theta_k^*)\|_2^2] \leq \sum_{l \in \mathcal{N}_k} \mathbb{E} [a_{lk}(i)] \mathbb{E} [\|\theta_{l,i} - \theta_k^*\|_2^2] = \sum_{l \in \mathcal{N}_k} a_{lk}^* \mathbb{E} [\|\theta_{l,i} - \theta_k^*\|_2^2],$$
% $$\mathbb{E} [\|\sum_{l \in \mathcal{N}_k} a_{lk}(i)  \nabla_{\theta_l} \ell_l^i(\theta_{l,i})) \|_2^2] \leq \sum_{l \in \mathcal{N}_k} \mathbb{E} [a_{lk}(i)] \mathbb{E} [ \|\nabla_{\theta_l} \ell_l^i(\theta_{l,i}))\|_2^2] = \sum_{l \in \mathcal{N}_k} a_{lk}^*  \mathbb{E} [ \|\nabla_{\theta_l} \ell_l^i(\theta_{l,i}))\|_2^2],$$
% $$
% \mathbb{E}\left[\left(\sum_{l \in \mathcal{N}_k} a_{lk}(i)  \nabla_{\theta_l} \ell_l^i(\theta_{l,i}) \right)^\top \left(\sum_{l \in \mathcal{N}_k} a_{lk}(i) (\theta_{l,i} - \theta_k^*) \right)\right] =  \left(\sum_{l \in \mathcal{N}_k} a_{lk}^* \mathbb{E} [ \nabla_{\theta_l} \ell_l^i(\theta_{l,i})]\right)^\top  \left(\sum_{l \in \mathcal{N}_k} a_{lk}^* \mathbb{E} [ (\theta_{l,i} - \theta_k^*)]\right)
% $$
\begin{equation*}
\begin{aligned}
     r_k(\theta_{k,i+1})  &= r_k\left(\sum_{l \in \mathcal{N}_k} a_{lk}(i)  \left({\theta}_{l,i} - \mu  \nabla_{\theta_l} \ell_{l}^i({\theta_{l,i}} ) \right) \right)
\end{aligned}
\end{equation*}
Given Jensen's inequality and taking expectations of the above equation, we have
\begin{equation*}
\begin{aligned}
     \mathbb{E} [r_k(\theta_{k,i+1})] \leq \sum_{l \in \mathcal{N}_k}  \mathbb{E} [a_{lk}(i)] \mathbb{E} \left[ r_k  \left(\hat{\theta}_{l,i} \right) \right] 
     = \sum_{l \in \mathcal{N}_k} a_{lk}^* \mathbb{E} \left[ r_k \left(\hat{\theta}_{l,i}  \right) \right] 
     \leq \mathbb{E} \left[ r_k \left(\hat{\theta}_{k,i}  \right) \right]
\end{aligned}
\end{equation*}
Next, we follow the convergence analysis of the SGD algorithm. Given the $L$-Lipschitz continuous gradient assumption of the risk functions, we have
\begin{equation*}
\begin{aligned}
    r_k \left(\hat{\theta}_{k,i}  \right) - r_k({\theta}_{k,i-1} ) &\leq  \nabla r_k ({\theta}_{k,i-1})^\top (\hat{\theta}_{k,i}  - {\theta}_{k,i-1}) + \frac{1}{2} L \| \hat{\theta}_{k,i}  - {\theta}_{k,i-1}\|_2^2 \\
    &= - \mu \nabla r_k ({\theta}_{k,i-1})^\top \nabla \ell_k^{i-1}(\theta_{k,i-1}) + \frac{1}{2} \mu^2 L \|\nabla \ell_k^{i-1}(\theta_{k,i-1})\|^2_2
\end{aligned}
\end{equation*}
We take the expected value of $\hat{\theta}_{k,i}$ with respect to the distribution given ${\theta}_{k,i-1}$ and obtain
\begin{equation*}
\begin{aligned}
  \mathbb{E}  \left[r_k \left(\hat{\theta}_{k,i}  \right) \right] - r_k({\theta}_{k,i-1} ) \leq   - \mu \nabla r_k ({\theta}_{k,i-1})^\top \mathbb{E} [\nabla  \ell_k^{i-1}(\theta_{k,i-1})] + \frac{1}{2} \mu^2 L \mathbb{E} [\|\nabla \ell_k^{i-1}(\theta_{k,i-1})\|^2_2]
\end{aligned}
\end{equation*}
Given the stochastic gradient $\nabla  \ell_k^{i}(\theta_{k,i})$ is an unbiased estimate of $\nabla r_k(\theta_{k,i})$, i.e., $\mathbb{E} [\nabla  \ell_k^{i-1}(\theta_{k,i-1})] =  \nabla r_k ({\theta}_{k,i-1})$, and restrict the variance of $\nabla \ell_k^{i-1}(\theta_{k,i-1})$, i.e.,
\begin{equation*}
    Var[\nabla \ell_k^{i}(\theta_{k,i})] = \mathbb{E}[\|\nabla \ell_k^{i}(\theta_{k,i})\|_2^2] - \|\mathbb{E}[\nabla \ell_k^{i}(\theta_{k,i})]\|_2^2 \leq \sigma_k^2,
\end{equation*}
we have $\mathbb{E}[\|\nabla \ell_k^{i}(\theta_{k,i})\|_2^2] \leq \|\mathbb{E}[\nabla \ell_k^{i}(\theta_{k,i})]\|_2^2 + \sigma_k^2 = \|\nabla r_k ({\theta}_{k,i})\|_2^2 + \sigma_k^2$. Hence, 
\begin{equation}\label{eq: expection of r_i minuus i-1}
\begin{aligned}
  \mathbb{E}  \left[r_k \left(\hat{\theta}_{k,i}  \right) \right] - r_k({\theta}_{k,i-1} ) &\leq   - \mu \|\nabla r_k ({\theta}_{k,i-1})\|_2^2 + \frac{1}{2} \mu^2 L \mathbb{E} [\|\nabla \ell_k^{i-1}(\theta_{k,i-1})\|^2_2]\\
  &\leq - \mu \|\nabla r_k ({\theta}_{k,i-1})\|_2^2 + \frac{1}{2} \mu^2 L \left(\|\nabla r_k ({\theta}_{k,i-1})\|_2^2 + \sigma_k^2\right)\\
  &= -\mu(1 - \frac{\mu L}{2}) \|\nabla r_k ({\theta}_{k,i-1})\|_2^2 + \frac{1}{2} \mu^2 L \sigma_k^2
\end{aligned}
\end{equation}
Given the strong convexity condition of $r_k$, there exists $m \leq L$ such that
\begin{equation*}
    \|\nabla r_k(\theta)\|_2^2 \geq 2m \left(r_k(\theta) - r_k^*\right) \text{ for all } \theta.
\end{equation*}
Therefore, \eqref{eq: expection of r_i minuus i-1} turns into
\begin{equation*}
    \mathbb{E}  \left[r_k \left(\hat{\theta}_{k,i}  \right) \right] - r_k({\theta}_{k,i-1} ) \leq   -2m \mu (1 - \frac{\mu L}{2})\left(r_k(\theta_{k,i-1}) - r_k^*\right) + \frac{1}{2} \mu^2 L \sigma_k^2
\end{equation*}
Subtracting $r_k^*$ from both sides and taking expectations, we have
\begin{equation*}
    \mathbb{E}  \left[r_k \left(\hat{\theta}_{k,i}  \right) - r_k^* \right] \leq  \left( 1 -2m \mu(1 - \frac{\mu L}{2}) \right)  \mathbb{E}\left[ \left(r_k(\theta_{k,i-1}) - r_k^*\right) \right] + \frac{1}{2} \mu^2 L \sigma_k^2
\end{equation*}
Subtracting the constant $\frac{\mu L \sigma_k^2}{2m(2 - \mu L)}$ from both sides, we obtain
\begin{equation*}
\begin{aligned}
      \mathbb{E}  \left[r_k \left(\hat{\theta}_{k,i}  \right) - r_k^* \right] - \frac{\mu L \sigma_k^2}{2m(2 - \mu L)} &\leq  \left( 1 -2m \mu (1 - \frac{\mu L}{2}) \right)  \mathbb{E}\left[ \left(r_k(\theta_{k,i-1}) - r_k^*\right) \right] + \frac{1}{2} \mu^2 L \sigma_k^2 - \frac{\mu L \sigma_k^2}{2m(2 - \mu L)} \\
      &= \left( 1 -2m \mu (1 - \frac{\mu L}{2}) \right) \left(  \mathbb{E}\left[ \left(r_k(\theta_{k,i-1}) - r_k^*\right) \right] - \frac{\mu L \sigma_k^2}{2m(2 - \mu L)}  \right)
\end{aligned}
\end{equation*}
Repeating through iteration $i$, we have
\begin{equation}\label{eq: contraction inequality}
\begin{aligned}
      \mathbb{E}  \left[r_k \left(\hat{\theta}_{k,i}  \right) - r_k^* \right] - \frac{\mu L \sigma_k^2}{2m(2 - \mu L)} \leq  \left( 1 -2m \mu (1 - \frac{\mu L}{2}) \right)^{i-1} \left(  \mathbb{E}\left[ \left(r_k(\theta_{k,1}) - r_k^*\right) \right] - \frac{\mu L \sigma_k^2}{2m(2 - \mu L)}  \right)
\end{aligned}
\end{equation}
Since $ 1 -2m \mu (1 - \frac{\mu L}{2}) = 1 + m \mu (L \mu - 2) \leq 1 + L\mu (L \mu - 2) = (L \mu - 1)^2$, by selecting fixed stepsize $\mu \in (0, \frac{2}{L}]$, $\left( 1 -2m \mu (1 - \frac{\mu L}{2}) \right) \in [0, 1)$, that guarantees $r_k\left(\hat{\theta}_{k,i}  \right)$ to converge towards $r_k^*$. And the expected optimality gap satisfies 
\begin{equation*}
\begin{aligned}
   \mathbb{E}  \left[r_k \left(\hat{\theta}_{k,i}  \right) - r_k^* \right] \leq&   \frac{\mu L \sigma_k^2}{2m(2 - \mu L)} +  \left( 1 -2m \mu (1 - \frac{\mu L}{2}) \right)^{i-1} \left(  \mathbb{E}\left[ \left(r_k(\theta_{k,1}) - r_k^*\right) \right] - \frac{\mu L \sigma_k^2}{2m(2 - \mu L)}  \right)\\
   \underrightarrow{i \rightarrow \infty}&   \frac{\mu L \sigma_k^2}{2m(2 - \mu L)}.
\end{aligned}
\end{equation*}


==> evaluation.tex <==
\section{Evaluation\footnote{Simulation details and supplementary results are given in Appendix \ref{app: Simulation Details and Supplementary Results}.}}
In this section, we evaluate the resilience of our proposed online weight adjustment rule \eqref{eq: filtering weight} 
and compare our method with the non-cooperative case, average weights, quadratic distance-based weights \eqref{eq: quadratic distance weight} (with $\tilde{\theta}_k^* = \theta_{k,i-1}$ and the same smoothing method used for \eqref{eq: filtering weight} ) 
using multiple distributed MTL datasets for both  regression and classification problems with and without the presence of Byzantine agents. 
Although our Byzantine resilient convergence analysis in Section \ref{sec: resilient convergence analysis} is specifical for convex models and stochastic gradient descent, we show that our weight assignment rule \eqref{eq: filtering weight} empirically perform well for non-convex models such as convolutional neural networks and mini-batch gradient descent too.
% \subsection{Datasets}
% \begin{itemize}[leftmargin=*]
% \item \textbf{Target Localization}


%     \item \textbf{Human Activity Recognition\footnote{https://archive.ics.uci.edu/ml/datasets/human+activity+recognition+using+smartphones}}\cite{DBLP:conf/esann/AnguitaGOPR13}:   Mobile phone sensor data (accelerometer and gyroscope) is collected from 30 individuals   performing one of six activities: \{walking, walking-upstairs, walking-downstairs, sitting, standing, lying-down\}. 
%   We model each individual as a separate task and use a fully-connected network to model the relationship among the 30 agents.
%   And predict the activities they perform using the  561-length feature vectors for each instance generated by the processed sensor signals.
   
   
%      \item \textbf{Digit classification}:
%     We consider a network of ten agents  performing the digit classification tasks.
% Five of the ten agents are access to the MNIST dataset\footnote{http://yann.lecun.com/exdb/mnist} \cite{lecun-mnisthandwrittendigit-2010}, and the other five are access to the synthetic digits dataset\footnote{https://www.kaggle.com/prasunroy/synthetic-digits} \cite{roy2018effects} that is composed by generated images of digits embedded on random backgrounds.
% All the images are preprocessed to be $28 \times 28 \times 1$ grayscale images.
% We model each agent as a separate task and use a fully-connected network to model the relationship among the 10 agents.
% And classify the digits $0-9$ using the preprocessed images.
% \figref{fig: Examples of the Digit classification dataset} are some preprocessed examples of the two datasets.
  
%     % \item \textbf{Facebook Comments Volume Prediction\footnote{https://archive.ics.uci.edu/ml/datasets/Facebook+Comment+Volume+Dataset} \cite{fbcommentVolumePrediction}}:
%     % Instances in this dataset contain features extracted from facebook posts. The task associated with the data is to predict how many comments the post will receive.
    
  
%     % \item \textbf{Parkinsons Telemonitoring\footnote{https://archive.ics.uci.edu/ml/datasets/Parkinsons+Telemonitoring}
%     % \cite{TelemonitoringParkinson}}:
% \end{itemize}



\subsection{Target Localization}\label{sec: target localization}
Target localization is a widely-studied linear regression example in distributed diffusion algorithms \cite{DBLP:conf/icassp/ChenRS14}.
We consider a network of 100 agents in the network as shown in \figref{fig: target localization network}. 
Agents estimate the location of one of the four targets  using linear regression with noisy streaming sensor data. Agents in the same color share the same target yet they do not know this group information beforehand.

\figref{fig: TL, no attack}-d shows the mean and range of the individual mean squared error loss of every normal agent's streaming data.
In the cases of no attack and 20 random selected Byzantine agents, we find loss-based weights \eqref{eq: filtering weight} perform better than the non-cooperative case --  the mean of the loss is smaller and the largest loss of normal agents (upper bound of the loss range) is smaller too, which validates the result indicated by \eqref{eq: resilient convergence  with improved learning error}. This implies the loss-based weights accurately learn the relationship among agents and those normal agents having a large regret in their measurements indeed benefit in cooperating with the other agents having a small regret. 
Even in the presence of  99 random selected Byzantine agents, the performance of the loss-based weights is close to that of the non-cooperative case, showing its resilience in MTL with arbitrary number of Byzantine agents.
Yet the average weights fail in convergence in all the cases. We also find the distance-based weights surprisingly perform badly in learning the relationship among agents and also fail in convergence in all the cases, which could be caused by the  small divergence among the targets.



\begin{figure}[!htb]
    \centering
\begin{minipage}{0.245\textwidth}
\begin{subfigure}{1\textwidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth, trim=1.5cm 1cm 1.5cm -0.2cm]{figure/network_attackerNum0.jpg} 
     \vspace{0.1cm}
  \caption{Network topology}
  \label{fig: target localization network}
\end{subfigure}
%   \label{fig:multi-task}
\end{minipage}
\begin{minipage}{0.745\textwidth}
\begin{minipage}{1\textwidth}
\centering
    \includegraphics[width=0.9\linewidth, trim=0cm 0.1cm -1cm 0cm]{figure/TL_legend_new.jpg}
\end{minipage}\\
\vspace{0cm}
\begin{minipage}{1\textwidth}
\begin{subfigure}{.325\textwidth}
  \centering
  % include first image
  \vspace{0.2cm}
  \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/TL_loss_no_attack.eps}  
  \caption{No attack}
  \label{fig: TL, no attack}
\end{subfigure}
\begin{subfigure}{.325\textwidth}
  \centering
  % include second image
    \vspace{0.2cm}
  \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/TL_loss_20attackers.eps}  
  \caption{20 Byzantine}
%   \label{fig:Byzantine}
\end{subfigure}
\begin{subfigure}{.325\textwidth}
  \centering
    \vspace{0.2cm}
  % include second image
  \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/TL_loss_99attackers.eps}  
  \caption{99 Byzantine}
   \label{fig: TL, 99 attackers}
\end{subfigure}
\end{minipage}%
\end{minipage}%
\caption{Target Localization: network topology and  loss of streaming data for normal agents.}
\label{fig: Target Localization: Network topology and average Loss for streaming data}
\end{figure}


\subsection{Human Activity Recognition}\label{sec: human action recognition}
Mobile phone sensor data (accelerometer and gyroscope)\footnote{https://archive.ics.uci.edu/ml/datasets/human+activity+recognition+using+smartphones} is collected from 30 individuals   performing one of six activities: \{walking, walking-upstairs, walking-downstairs, sitting, standing, lying-down\}. 
The goal is to predict the activities they perform using the  561-length feature vectors for each instance generated by the processed sensor signals \cite{DBLP:conf/esann/AnguitaGOPR13}.
We model each individual as a separate task and use a complete graph to model the network topology among the 30 agents.
We randomly split the data into 75\% training and 25\% testing for each agent and use a linear model as the prediction function with cross-entropy-loss.

\begin{figure}[ht]
\centering
\vspace{0.1cm}
\begin{subfigure}{0.495\textwidth}
  \centering
  \begin{minipage}{.48\textwidth}
  \centering
    \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/HAR_range_loss_test_noattack.eps}  
  \end{minipage}
    \begin{minipage}{.48\textwidth}
  \centering
    \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/HAR_range_acc_test_noattack.eps}  
  \end{minipage}
\caption{No attack}
\end{subfigure}
\begin{subfigure}{0.495\textwidth}
  \centering
  \begin{minipage}{.48\textwidth}
  \centering
    \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/HAR_range_loss_test_attack_10.eps}  
  \end{minipage}
  % include first image
  \begin{minipage}{.48\textwidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/HAR_range_acc_test_attack_10.eps}  
%   \label{fig:multi-task}
\end{minipage}
\caption{10 Byzantine agents}
\end{subfigure}
% \begin{subfigure}{0.325\textwidth}
%   \centering
%   \begin{minipage}{.48\textwidth}
%   \centering
%     \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/HAR_range_loss_test_attack_99.eps}  
%   \end{minipage}
%   % include first image
%   \begin{minipage}{.48\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/HAR_range_acc_test_attack_99.eps}  
% %   \label{fig:multi-task}
% \end{minipage}
% \caption{29 Byzantine agents}
% \end{subfigure}
\caption{Human Action Recognition: average testing loss and  accuracy for normal agents.}
\label{fig: har test}
\end{figure}

The mean and range of the individual average testing loss and accuracy of every normal agent in the case of no attack, and with 10 randomly selected Byzantine agents, is presented in \figref{fig: har test} (legend is the same as in \figref{fig: Target Localization: Network topology and average Loss for streaming data}).
% (Same results for training can be found in \figref{fig: har train} in Appendix, legend is the same as in \figref{fig: Target Localization: Network topology and average Loss for streaming data}).
We find overall the loss-based weights \eqref{eq: filtering weight} outperforms  the non-cooperative case and the other combination rules  in all the cases, with respect to the mean and range of the average loss and accuracy. 
%And even when 29 of the 30 agents are Byzantine, the loss-based weights can still resiliently converge and performs close to the non-cooperative case.

% In the case of no cooperation, since 10 of the 30 tasks are training their model based on limited data, they are pruned to overfit their models such that they have a better average loss and prediction accuracy on the training data than on the testing data. The cooperation using the loss-based rule help correct such overfitting -- overfitted models will be tuned by non-overfitted models, yet non-overfitted models will not be influenced by the overfitted models.
% However, the average rule that simply averages over the overfitted and non-overfitted data will make the non-overfitted models also be influenced by the overfitted models. As a result, the average rule performs worse than the non-cooperative case.

% By introducing one Byzantine agent that always sends a model with very small noisy elements for each dimension, we find the loss-based rule is resilient as it still performs better than the non-cooperative case, yet the average rule has been attacked to have a large loss and low prediction accuracy.

\subsection{Handwritten Digit Classification}\label{sec: Digit classification}
We consider a network of ten agents  performing the digit classification tasks.
Five of the ten agents are access to the MNIST dataset\footnote{http://yann.lecun.com/exdb/mnist}  \cite{lecun-mnisthandwrittendigit-2010} (group 1), and the other five are access to the synthetic digits dataset\footnote{https://www.kaggle.com/prasunroy/synthetic-digits} \cite{roy2018effects} (group 2) that is composed by generated images of digits embedded on random backgrounds.
All the images are preprocessed to be $28 \times 28 \times 1$ grayscale images.
We model each agent as a separate task and use a complete graph to  model the network topology among the ten agents.
% We classify the digits $0-9$ using the preprocessed images.
% \figref{fig: Examples of the Digit classification dataset} in Appendix are some preprocessed examples of the two datasets.
% We refer to the 5 agents for the MNIST dataset as group 1 and the other 5 agents for the synthetic digits dataset as group 2. 
However, agents do not know which of its neighbors are performing the same task as itself.
% (or which of the neighbors are access to the same dataset as itself).
% For each group, we consider agents are access to uneven sizes of training data.
% For each agent, we randomly pass $200-2000$ training data and $400$ testing data from the corresponding dataset for each epoch. Since some of the agents are access to limited training data, they are prone to overfitting or learn slowly if without cooperation.
We use a CNN model of the same architecture for each agent and cross-entropy-loss.
% and use mini-batch gradient descent with batch size of $64$ and step-sizes (learning rate) $\mu_k = 0.001$ and forgetting factor $\nu_k = 0.05$ for all the normal agents.

We plot the results separately for the two groups. 
The mean and range of the individual average testing loss and accuracy of every normal agent in the case of no attack, and with 2 randomly selected Byzantine agents (one for each group), 
% and with 8 randomly selected Byzantine agents (four for each group), 
is presented in 
% \figref{fig: MNist test} for agents in group 1 and 
\figref{fig: synthetic test} for agents in group 2 
% (Same results for training can be found in \figref{fig: MNist train} and \figref{fig: synthetic train} in Appendix, 
(legend is the same as in \figref{fig: Target Localization: Network topology and average Loss for streaming data}).
% It is obvious from the results that agents in group 1 have  better learning performance than agents in group 2 since the synthetic digit classification is more challenging than the MNIST digit classification.
% Yet using the loss-based weights, agents are able to correctly identify the neighbors estimating the same task and use the cooperation to benefit their own learning performance. 
% The loss-based weights still outperform the other combination rules in all the cases, with respect to the mean and range of the average loss and accuracy. And even when 8 of the 10 agents are Byzantine (only one normal agent for each group), the loss-based weights can still resiliently converge and performs close to the non-cooperative case.





\begin{figure}[ht]
\centering
% \begin{minipage}{1\textwidth}
% \centering
%     \includegraphics[width=0.7\linewidth, trim=0cm -0.4cm -1cm 0cm]{figure/TL_legend_new.jpg}
% \end{minipage}\\
% \vspace{0.1cm}
\begin{subfigure}{0.495\textwidth}
  \centering
  \begin{minipage}{.48\textwidth}
  \centering
    \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/synthetic_range_loss_test_noattack.eps}  
  \end{minipage}
  % include first image
  \begin{minipage}{.48\textwidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/synthetic_range_acc_test_noattack.eps}  
%   \label{fig:multi-task}
\end{minipage}
\caption{No attack}
\end{subfigure}
\begin{subfigure}{0.495\textwidth}
  \centering
  \begin{minipage}{.48\textwidth}
  \centering
    \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/synthetic_range_loss_test_attack_2.eps}  
  \end{minipage}
  % include first image
  \begin{minipage}{.48\textwidth}
  \centering
  % include first image
  \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/synthetic_range_acc_test_attack_2.eps}  
%   \label{fig:multi-task}
\end{minipage}
\caption{2 Byzantine agents}
\end{subfigure}
% \begin{subfigure}{0.325\textwidth}
%   \centering
%   \begin{minipage}{.48\textwidth}
%   \centering
%     \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/synthetic_range_loss_test_attack_8.eps}  
%   \end{minipage}
%   % include first image
%   \begin{minipage}{.48\textwidth}
%   \centering
%   % include first image
%   \includegraphics[width=1\linewidth, trim=1cm 0cm 0cm 1cm]{figure/synthetic_range_acc_test_attack_8.eps}  
% %   \label{fig:multi-task}
% \end{minipage}
% \caption{8 Byzantine agents}
% \end{subfigure}
\caption{Digit classification: average testing loss and  accuracy for normal agents in group 2.}
\label{fig: synthetic test}
\end{figure}


